A New Approach for Active Automata Learning Based on Apartness

We present $L^{\#}$, a new and simple approach to active automata learning. Instead of focusing on equivalence of observations, like the $L^{\ast}$ algorithm and its descendants, $L^{\#}$ takes a different perspective: it tries to establish apartness, a constructive form of inequality. $L^{\#}$ does not require auxiliary notions such as observation tables or discrimination trees, but operates directly on tree-shaped automata. $L^{\#}$ has the same asymptotic query and symbol complexities as the best existing learning algorithms, but we show that adaptive distinguishing sequences can be naturally integrated to boost the performance of $L^{\#}$ in practice. Experiments with a prototype implementation, written in Rust, suggest that $L^{\#}$ is competitive with existing algorithms.

==> optimizations.tex <==




\section{Further Optimizations}
\label{sec:opt}
In this section, we describe some further optimizations that we have not yet implemented but that can be easily used to improve the performance of $\lsharp$.


\paragraph{Adaptive distinguishing sequences}
In the version of $\lsharp$ that we describe in this paper and implemented in Rust, adaptive distinguishing sequences are used in rule (R2) but not in rule (R3). The reason is that although the ADS's that we compute maximize the expected number of new apartness pairs, it may occur that an ADS-query does not produce a new apartness pair.  For rule (R2) this is not a problem (as a state is added to the frontier the norm will increase anyway), but when we replace the output query in rule (R3) by $\mathsf{access}(q) \; \Ads(\{ r \in S \mid \neg (q \# r) \})$, then there is no guarantee that the norm will increase. But what we could do, of course, is first try the ADS and resort to separating sequences in the rare cases where no new apartness pair is created.  This simple optimization would definitely reduce the total number of queries.

A potential problem with using ADS's is that their depth may be very high. Therefore, in order to reduce the expected number of input symbols, it may be better to impose a bound on the depth of the ADS's that are used.

As long as the observation tree is not too big we may compute the optimal ADS directly from the observation tree. However, for Mealy machines with many states (say $> 1000$), this may no longer be feasible.
A possible optimization would be to use instead an ADS that is computed using the algorithm of  \citet{LYa94}.
When the learner has constructed a new hypothesis $\Hyp$, it computes its ADS and does a corresponding output query for all states of basis $S$. If the results are inconsistent with $\Hyp$, this means it has found a new counterexample.
During construction of the next hypothesis, whenever the learner explore a new state $q$ on the frontier it first runs an output query with the ADS, to set $q$ apart from as many states in the basis as possible.
This optimization requires $\bigO(n^2)$ additional queries and will not affect the asymptotic query complexity of $\lsharp$. However, in practice this approach will be more scalable than computing the optimal ADS directly from the observation tree.

\paragraph{Minimal separating sequences}
It is well-known that the length of a minimal separating sequence for states $q$ and $q'$ for a minimal Mealy machine $\M$ with $n$ states is at most $n - 1$ \cite{Mo56}.  An efficient $\bigO(k n \log n)$ time algorithm for computing minimal separating sequences for all pairs of states of a Mealy machine has been proposed by \cite{SmetsersMJ16}. 
We may use these minimal separating sequences to optimize the performance of $\lsharp$.
%
%
%
%
%
%
%
%
%
When a hypothesis $\Hyp$ is consistent with the observation tree $\Obs$ then it is minimal.
Thus we may compute minimal separating sequences for all pairs of states.
Whenever, for two states $q$ and $q'$ of $\Hyp$, the minimal witness $\sigma$ for $q \# q'$ in $\Obs$ is longer then the minimal separating sequence $\rho$ in $\Hyp$, we pose output queries $\mathsf{access}(q) \rho$ and $\mathsf{access}(q') \rho$.  If the output in response to $\rho$ from $q$ differs from the output in response to $\rho$ from $q'$, then we have obtained a short witness for $q \; \# \; q'$ in $\Obs$. Otherwise, we have obtained a short counterexample for hypothesis $\Hyp$.
This optimization requires at most $\bigO(n^2)$ additional output queries and will thus not affect the asymptotic query complexity of $\lsharp$.








==> table_full_1.tex <==
% Warning: do not edit this file manually!
%
%
\begin{tabular}{@{}@{}l@{\hspace{1mm}}l@{}c@{}l@{}c@{}r@{}c@{}r@{\hspace{1mm}}r@{}c@{}r@{\hspace{1mm}}r@{}c@{}r@{}@{}}
\toprule%
\multicolumn{2}{@{}l@{}}{Model}
&\hspace*{2mm}&
\multicolumn{1}{@{}l@{}}{Algo-}
&\hspace*{2mm}&
\multicolumn{1}{@{}l@{}}{}
&\hspace*{2mm}&
\multicolumn{2}{@{}l@{}}{Learn-}
&\hspace*{2mm}&
\multicolumn{2}{@{}l@{}}{Test-}
&\hspace*{2mm}&
\multicolumn{1}{@{}l@{}}{}
\\
\cline{1-2}
%
%
\cline{8-9}
\cline{11-12}
%
\\[-4pt]
$n$
&
$k$
&
&
rithm
&
&
EQs
&
&
Inputs
&
Resets
&
&
Inputs
&
Resets
&
&
Total
\\
\midrule
\multicolumn{2}{@{}l@{}}{4\_learnresult\_SecureCodeAut\_fix}&&$\lsharp$&&3.00&&484.35&146.36&&194.60&17.87&&843.18\\
&&&$\lsharp_{\Ads}$&&3.00&&\bestvalue{322.58}&\bestvalue{96.04}&&207.26&18.13&&\bestvalue{644.01}\\
$n$ = 4&$k$ = 14&&\texttt{TTT}&&2.95&&495.57&149.24&&210.96&16.78&&872.55\\
&&&\texttt{ADT}&&\bestvalue{2.93}&&477.73&115.56&&201.74&16.55&&811.58\\
&&&\texttt{RS}&&2.99&&1214.37&132.19&&\bestvalue{170.30}&\bestvalue{14.47}&&1531.33\\
\arrayrulecolor{black!20}\hline\arrayrulecolor{black}
\multicolumn{2}{@{}l@{}}{ASN\_learnresult\_SecureCodeAut\_fix}&&$\lsharp$&&3.00&&485.74&146.43&&225.31&19.89&&877.37\\
&&&$\lsharp_{\Ads}$&&3.00&&\bestvalue{327.35}&\bestvalue{96.74}&&206.05&17.67&&\bestvalue{647.81}\\
$n$ = 4&$k$ = 14&&\texttt{TTT}&&2.94&&495.52&149.38&&216.96&17.21&&879.07\\
&&&\texttt{ADT}&&2.92&&458.28&110.40&&163.00&14.21&&745.89\\
&&&\texttt{RS}&&\bestvalue{2.91}&&1252.11&127.60&&\bestvalue{159.23}&\bestvalue{13.15}&&1552.09\\
\arrayrulecolor{black!20}\hline\arrayrulecolor{black}
\multicolumn{2}{@{}l@{}}{1\_learnresult\_MasterCard\_fix}&&$\lsharp$&&\bestvalue{3.00}&&728.63&201.45&&\bestvalue{81.59}&\bestvalue{9.19}&&\bestvalue{1020.86}\\
&&&$\lsharp_{\Ads}$&&3.75&&\bestvalue{576.70}&\bestvalue{141.09}&&359.43&29.03&&1106.25\\
$n$ = 5&$k$ = 15&&\texttt{TTT}&&3.42&&620.95&187.46&&227.21&18.15&&1053.77\\
&&&\texttt{ADT}&&3.71&&818.83&165.08&&449.64&34.49&&1468.04\\
&&&\texttt{RS}&&3.32&&2347.76&196.97&&344.27&26.32&&2915.32\\
\arrayrulecolor{black!20}\hline\arrayrulecolor{black}
\multicolumn{2}{@{}l@{}}{OpenSSL\_1.0.1j\_client\_regular}&&$\lsharp$&&6.00&&439.25&114.64&&2866.97&218.78&&3639.64\\
&&&$\lsharp_{\Ads}$&&5.91&&\bestvalue{200.30}&\bestvalue{56.01}&&2244.26&175.18&&2675.75\\
$n$ = 6&$k$ = 7&&\texttt{TTT}&&\bestvalue{4.35}&&320.91&92.23&&\bestvalue{1679.45}&\bestvalue{128.02}&&\bestvalue{2220.61}\\
&&&\texttt{ADT}&&4.89&&475.37&89.39&&2131.04&161.65&&2857.45\\
&&&\texttt{RS}&&4.60&&1868.79&165.97&&1979.22&149.00&&4162.98\\
\arrayrulecolor{black!20}\hline\arrayrulecolor{black}
\multicolumn{2}{@{}l@{}}{OpenSSL\_1.0.1l\_client\_regular}&&$\lsharp$&&6.00&&441.21&115.42&&2576.04&198.39&&3331.06\\
&&&$\lsharp_{\Ads}$&&5.90&&\bestvalue{199.65}&\bestvalue{55.88}&&2057.69&159.52&&2472.74\\
$n$ = 6&$k$ = 7&&\texttt{TTT}&&4.54&&295.63&85.73&&1859.69&141.00&&\bestvalue{2382.05}\\
&&&\texttt{ADT}&&4.89&&465.76&88.15&&2446.06&182.21&&3182.18\\
&&&\texttt{RS}&&\bestvalue{4.49}&&1915.47&161.12&&\bestvalue{1838.95}&\bestvalue{139.71}&&4055.25\\
\arrayrulecolor{black!20}\hline\arrayrulecolor{black}
\multicolumn{2}{@{}l@{}}{OpenSSL\_1.0.2\_client\_regular}&&$\lsharp$&&6.00&&440.58&114.76&&2442.08&188.35&&3185.77\\
&&&$\lsharp_{\Ads}$&&5.93&&\bestvalue{201.51}&\bestvalue{56.45}&&2197.54&172.05&&2627.55\\
$n$ = 6&$k$ = 7&&\texttt{TTT}&&5.31&&312.40&89.52&&\bestvalue{1896.67}&145.52&&\bestvalue{2444.11}\\
&&&\texttt{ADT}&&4.92&&447.98&87.94&&2237.95&167.92&&2941.79\\
&&&\texttt{RS}&&\bestvalue{4.60}&&1727.94&165.39&&1899.77&\bestvalue{143.42}&&3936.52\\
\arrayrulecolor{black!20}\hline\arrayrulecolor{black}
\multicolumn{2}{@{}l@{}}{RSA\_BSAFE\_Java\_6.1.1\_server\_regular}&&$\lsharp$&&4.94&&419.53&112.52&&3444.36&264.15&&4240.56\\
&&&$\lsharp_{\Ads}$&&4.95&&\bestvalue{198.28}&\bestvalue{56.81}&&3412.44&261.89&&3929.42\\
$n$ = 6&$k$ = 8&&\texttt{TTT}&&4.84&&322.00&94.00&&3201.54&239.90&&3857.44\\
&&&\texttt{ADT}&&4.55&&369.82&79.67&&2777.73&213.04&&\bestvalue{3440.26}\\
&&&\texttt{RS}&&\bestvalue{4.50}&&1840.03&181.51&&\bestvalue{2631.52}&\bestvalue{201.02}&&4854.08\\
\arrayrulecolor{black!20}\hline\arrayrulecolor{black}
\multicolumn{2}{@{}l@{}}{miTLS\_0.1.3\_server\_regular}&&$\lsharp$&&4.00&&579.69&154.13&&\bestvalue{1329.16}&\bestvalue{104.97}&&2167.95\\
&&&$\lsharp_{\Ads}$&&4.35&&\bestvalue{320.61}&87.79&&1609.79&128.98&&2147.17\\
$n$ = 6&$k$ = 8&&\texttt{TTT}&&3.99&&481.64&136.55&&1377.39&105.62&&\bestvalue{2101.20}\\
&&&\texttt{ADT}&&4.27&&375.66&\bestvalue{82.58}&&2227.62&170.22&&2856.08\\
&&&\texttt{RS}&&\bestvalue{3.97}&&1703.94&156.19&&1945.37&146.89&&3952.39\\
\arrayrulecolor{black!20}\hline\arrayrulecolor{black}
\multicolumn{2}{@{}l@{}}{10\_learnresult\_MasterCard\_fix}&&$\lsharp$&&4.00&&894.32&229.38&&\bestvalue{2399.60}&\bestvalue{177.44}&&3700.74\\
&&&$\lsharp_{\Ads}$&&4.00&&\bestvalue{668.80}&\bestvalue{163.13}&&2673.32&195.45&&\bestvalue{3700.70}\\
$n$ = 6&$k$ = 14&&\texttt{TTT}&&\bestvalue{3.95}&&895.90&229.52&&3278.16&238.56&&4642.14\\
&&&\texttt{ADT}&&4.35&&947.33&199.58&&2871.02&208.77&&4226.70\\
&&&\texttt{RS}&&4.14&&3681.22&288.22&&2838.96&206.23&&7014.63\\
\arrayrulecolor{black!20}\hline\arrayrulecolor{black}
\multicolumn{2}{@{}l@{}}{4\_learnresult\_MAESTRO\_fix}&&$\lsharp$&&4.00&&897.31&229.19&&3115.73&225.96&&4468.19\\
&&&$\lsharp_{\Ads}$&&4.00&&\bestvalue{663.51}&\bestvalue{162.87}&&3035.95&223.70&&\bestvalue{4086.03}\\
$n$ = 6&$k$ = 14&&\texttt{TTT}&&\bestvalue{3.93}&&892.34&229.45&&3152.39&228.05&&4502.23\\
&&&\texttt{ADT}&&4.45&&941.28&196.62&&2833.00&203.47&&4174.37\\
&&&\texttt{RS}&&4.18&&3446.26&291.62&&\bestvalue{2509.68}&\bestvalue{179.91}&&6427.47\\
\bottomrule
\end{tabular}


==> table_full_2.tex <==
% Warning: do not edit this file manually!
%
%
\begin{tabular}{@{}@{}l@{\hspace{1mm}}l@{}c@{}l@{}c@{}r@{}c@{}r@{\hspace{1mm}}r@{}c@{}r@{\hspace{1mm}}r@{}c@{}r@{}@{}}
\toprule%
\multicolumn{2}{@{}l@{}}{Model}
&\hspace*{2mm}&
\multicolumn{1}{@{}l@{}}{Algo-}
&\hspace*{2mm}&
\multicolumn{1}{@{}l@{}}{}
&\hspace*{2mm}&
\multicolumn{2}{@{}l@{}}{Learn-}
&\hspace*{2mm}&
\multicolumn{2}{@{}l@{}}{Test-}
&\hspace*{2mm}&
\multicolumn{1}{@{}l@{}}{}
\\
\cline{1-2}
%
%
\cline{8-9}
\cline{11-12}
%
\\[-4pt]
$n$
&
$k$
&
&
rithm
&
&
EQs
&
&
Inputs
&
Resets
&
&
Inputs
&
Resets
&
&
Total
\\
\midrule
\multicolumn{2}{@{}l@{}}{4\_learnresult\_PIN\_fix}&&$\lsharp$&&4.00&&894.15&229.08&&\bestvalue{2379.98}&\bestvalue{176.20}&&\bestvalue{3679.41}\\
&&&$\lsharp_{\Ads}$&&4.00&&\bestvalue{672.03}&\bestvalue{163.36}&&2761.73&203.21&&3800.33\\
$n$ = 6&$k$ = 14&&\texttt{TTT}&&\bestvalue{3.97}&&895.99&229.75&&2979.36&216.20&&4321.30\\
&&&\texttt{ADT}&&4.39&&905.19&189.10&&2687.80&195.58&&3977.67\\
&&&\texttt{RS}&&4.16&&3512.37&289.47&&2476.66&179.00&&6457.50\\
\arrayrulecolor{black!20}\hline\arrayrulecolor{black}
\multicolumn{2}{@{}l@{}}{ASN\_learnresult\_MAESTRO\_fix}&&$\lsharp$&&4.00&&895.02&228.81&&3092.95&224.88&&4441.66\\
&&&$\lsharp_{\Ads}$&&4.00&&\bestvalue{664.85}&\bestvalue{162.74}&&2587.53&189.71&&\bestvalue{3604.83}\\
$n$ = 6&$k$ = 14&&\texttt{TTT}&&\bestvalue{3.99}&&892.60&229.66&&3469.10&252.07&&4843.43\\
&&&\texttt{ADT}&&4.47&&927.69&196.79&&3159.81&228.45&&4512.74\\
&&&\texttt{RS}&&4.12&&3418.29&285.89&&\bestvalue{2318.70}&\bestvalue{167.20}&&6190.08\\
\arrayrulecolor{black!20}\hline\arrayrulecolor{black}
\multicolumn{2}{@{}l@{}}{Rabo\_learnresult\_MAESTRO\_fix}&&$\lsharp$&&4.00&&900.82&229.37&&3015.36&220.35&&4365.90\\
&&&$\lsharp_{\Ads}$&&4.00&&\bestvalue{667.36}&\bestvalue{162.94}&&\bestvalue{2689.37}&196.94&&\bestvalue{3716.61}\\
$n$ = 6&$k$ = 14&&\texttt{TTT}&&\bestvalue{3.97}&&896.20&229.75&&3562.85&255.31&&4944.11\\
&&&\texttt{ADT}&&4.46&&930.73&192.82&&3050.85&220.12&&4394.52\\
&&&\texttt{RS}&&4.06&&3081.30&280.15&&2703.82&\bestvalue{195.80}&&6261.07\\
\arrayrulecolor{black!20}\hline\arrayrulecolor{black}
\multicolumn{2}{@{}l@{}}{Rabo\_learnresult\_SecureCode\_Aut\_fix}&&$\lsharp$&&4.00&&1016.16&251.29&&1531.42&111.57&&2910.44\\
&&&$\lsharp_{\Ads}$&&4.00&&\bestvalue{737.42}&\bestvalue{174.67}&&1487.81&107.97&&\bestvalue{2507.87}\\
$n$ = 6&$k$ = 15&&\texttt{TTT}&&3.92&&999.53&249.37&&1475.98&105.90&&2830.78\\
&&&\texttt{ADT}&&4.23&&1196.91&243.05&&2485.44&171.59&&4096.99\\
&&&\texttt{RS}&&\bestvalue{3.69}&&3221.53&266.03&&\bestvalue{1257.26}&\bestvalue{89.63}&&4834.45\\
\arrayrulecolor{black!20}\hline\arrayrulecolor{black}
\multicolumn{2}{@{}l@{}}{OpenSSL\_1.0.2\_server\_regular}&&$\lsharp$&&5.64&&491.62&135.43&&2523.07&195.46&&3345.58\\
&&&$\lsharp_{\Ads}$&&6.55&&\bestvalue{335.43}&\bestvalue{89.22}&&2543.01&194.99&&\bestvalue{3162.65}\\
$n$ = 7&$k$ = 7&&\texttt{TTT}&&5.70&&475.28&137.84&&2398.72&182.75&&3194.59\\
&&&\texttt{ADT}&&5.59&&557.41&112.91&&2445.53&184.98&&3300.83\\
&&&\texttt{RS}&&\bestvalue{4.89}&&1969.57&201.53&&\bestvalue{1673.30}&\bestvalue{128.78}&&3973.18\\
\arrayrulecolor{black!20}\hline\arrayrulecolor{black}
\multicolumn{2}{@{}l@{}}{GnuTLS\_3.3.12\_client\_regular}&&$\lsharp$&&4.92&&562.16&149.79&&4777.83&342.42&&5832.20\\
&&&$\lsharp_{\Ads}$&&4.98&&\bestvalue{244.03}&\bestvalue{69.06}&&3853.00&279.03&&4445.12\\
$n$ = 7&$k$ = 8&&\texttt{TTT}&&4.84&&397.92&116.05&&3395.21&247.80&&\bestvalue{4156.98}\\
&&&\texttt{ADT}&&\bestvalue{4.61}&&455.24&97.04&&3490.28&251.97&&4294.53\\
&&&\texttt{RS}&&4.68&&2496.24&220.92&&\bestvalue{3202.27}&\bestvalue{231.87}&&6151.30\\
\arrayrulecolor{black!20}\hline\arrayrulecolor{black}
\multicolumn{2}{@{}l@{}}{GnuTLS\_3.3.12\_server\_regular}&&$\lsharp$&&4.99&&563.83&149.99&&\bestvalue{2865.63}&214.65&&3794.10\\
&&&$\lsharp_{\Ads}$&&4.92&&\bestvalue{244.02}&\bestvalue{68.82}&&3877.60&280.35&&4470.79\\
$n$ = 7&$k$ = 8&&\texttt{TTT}&&5.65&&427.35&122.42&&4400.93&319.48&&5270.18\\
&&&\texttt{ADT}&&\bestvalue{4.67}&&448.58&98.50&&2882.06&\bestvalue{211.32}&&\bestvalue{3640.46}\\
&&&\texttt{RS}&&4.74&&2397.88&224.18&&3073.54&223.68&&5919.28\\
\arrayrulecolor{black!20}\hline\arrayrulecolor{black}
\multicolumn{2}{@{}l@{}}{NSS\_3.17.4\_client\_regular}&&$\lsharp$&&5.95&&631.47&144.44&&4239.68&324.29&&5339.88\\
&&&$\lsharp_{\Ads}$&&5.92&&\bestvalue{378.23}&\bestvalue{86.18}&&4734.30&359.43&&5558.14\\
$n$ = 7&$k$ = 8&&\texttt{TTT}&&4.92&&402.21&106.06&&\bestvalue{2687.59}&\bestvalue{203.47}&&\bestvalue{3399.33}\\
&&&\texttt{ADT}&&4.85&&477.09&94.10&&3204.14&244.10&&4019.43\\
&&&\texttt{RS}&&\bestvalue{4.70}&&2335.73&220.75&&3216.35&240.62&&6013.45\\
\arrayrulecolor{black!20}\hline\arrayrulecolor{black}
\multicolumn{2}{@{}l@{}}{Volksbank\_learnresult\_MAESTRO\_fix}&&$\lsharp$&&4.90&&1522.08&342.88&&407.92&31.60&&2304.48\\
&&&$\lsharp_{\Ads}$&&4.79&&\bestvalue{874.04}&\bestvalue{192.04}&&409.50&32.33&&\bestvalue{1507.91}\\
$n$ = 7&$k$ = 14&&\texttt{TTT}&&3.70&&1177.17&273.76&&415.49&29.48&&1895.90\\
&&&\texttt{ADT}&&3.79&&1412.84&233.27&&347.55&24.04&&2017.70\\
&&&\texttt{RS}&&\bestvalue{3.14}&&2683.45&230.76&&\bestvalue{141.85}&\bestvalue{10.72}&&3066.78\\
\arrayrulecolor{black!20}\hline\arrayrulecolor{black}
\multicolumn{2}{@{}l@{}}{NSS\_3.17.4\_server\_regular}&&$\lsharp$&&5.56&&599.68&150.57&&4424.54&334.87&&5509.66\\
&&&$\lsharp_{\Ads}$&&5.40&&\bestvalue{288.12}&\bestvalue{76.45}&&4227.87&323.47&&4915.91\\
$n$ = 8&$k$ = 8&&\texttt{TTT}&&5.15&&561.69&150.21&&\bestvalue{2693.04}&\bestvalue{205.19}&&\bestvalue{3610.13}\\
&&&\texttt{ADT}&&5.48&&570.48&118.95&&3918.63&293.35&&4901.41\\
&&&\texttt{RS}&&\bestvalue{4.98}&&2974.54&267.54&&3397.81&254.65&&6894.54\\
\arrayrulecolor{black!20}\hline\arrayrulecolor{black}
\multicolumn{2}{@{}l@{}}{RSA\_BSAFE\_C\_4.0.4\_server\_regular}&&$\lsharp$&&4.93&&626.48&169.71&&3151.88&215.60&&4163.67\\
&&&$\lsharp_{\Ads}$&&5.52&&\bestvalue{346.25}&\bestvalue{87.92}&&2944.89&201.13&&\bestvalue{3580.19}\\
$n$ = 9&$k$ = 8&&\texttt{TTT}&&5.53&&526.40&149.94&&5109.60&330.75&&6116.69\\
&&&\texttt{ADT}&&4.35&&764.37&140.03&&2948.31&197.35&&4050.06\\
&&&\texttt{RS}&&\bestvalue{4.24}&&2660.90&245.70&&\bestvalue{2549.10}&\bestvalue{173.86}&&5629.56\\
\bottomrule
\end{tabular}


==> table_full_3.tex <==
% Warning: do not edit this file manually!
%
%
\begin{tabular}{@{}@{}l@{\hspace{1mm}}l@{}c@{}l@{}c@{}r@{}c@{}r@{\hspace{1mm}}r@{}c@{}r@{\hspace{1mm}}r@{}c@{}r@{}@{}}
\toprule%
\multicolumn{2}{@{}l@{}}{Model}
&\hspace*{2mm}&
\multicolumn{1}{@{}l@{}}{Algo-}
&\hspace*{2mm}&
\multicolumn{1}{@{}l@{}}{}
&\hspace*{2mm}&
\multicolumn{2}{@{}l@{}}{Learn-}
&\hspace*{2mm}&
\multicolumn{2}{@{}l@{}}{Test-}
&\hspace*{2mm}&
\multicolumn{1}{@{}l@{}}{}
\\
\cline{1-2}
%
%
\cline{8-9}
\cline{11-12}
%
\\[-4pt]
$n$
&
$k$
&
&
rithm
&
&
EQs
&
&
Inputs
&
Resets
&
&
Inputs
&
Resets
&
&
Total
\\
\midrule
\multicolumn{2}{@{}l@{}}{OpenSSL\_1.0.2\_client\_full}&&$\lsharp$&&7.90&&1233.59&307.07&&26255.54&1824.25&&29620.45\\
&&&$\lsharp_{\Ads}$&&7.82&&\bestvalue{690.52}&\bestvalue{164.74}&&25024.71&1744.82&&27624.79\\
$n$ = 9&$k$ = 10&&\texttt{TTT}&&\bestvalue{5.98}&&735.55&204.92&&\bestvalue{21819.77}&\bestvalue{1537.01}&&\bestvalue{24297.25}\\
&&&\texttt{ADT}&&6.24&&965.68&198.12&&25715.06&1772.96&&28651.82\\
&&&\texttt{RS}&&7.05&&6788.28&562.07&&22996.72&1565.32&&31912.39\\
\arrayrulecolor{black!20}\hline\arrayrulecolor{black}
\multicolumn{2}{@{}l@{}}{GnuTLS\_3.3.12\_client\_full}&&$\lsharp$&&8.24&&1445.77&356.32&&\bestvalue{37675.94}&\bestvalue{2645.50}&&\bestvalue{42123.53}\\
&&&$\lsharp_{\Ads}$&&8.17&&\bestvalue{548.64}&\bestvalue{145.02}&&39712.47&2776.01&&43182.14\\
$n$ = 9&$k$ = 12&&\texttt{TTT}&&7.82&&832.63&233.49&&55244.09&3674.93&&59985.14\\
&&&\texttt{ADT}&&\bestvalue{6.87}&&1005.87&214.65&&38305.05&2653.84&&42179.41\\
&&&\texttt{RS}&&7.61&&9013.67&735.01&&43531.60&2979.22&&56259.50\\
\arrayrulecolor{black!20}\hline\arrayrulecolor{black}
\multicolumn{2}{@{}l@{}}{GnuTLS\_3.3.12\_server\_full}&&$\lsharp$&&5.55&&1367.74&336.92&&11819.63&825.78&&14350.07\\
&&&$\lsharp_{\Ads}$&&5.72&&\bestvalue{499.24}&\bestvalue{133.13}&&9782.28&682.94&&11097.59\\
$n$ = 9&$k$ = 12&&\texttt{TTT}&&5.87&&791.64&224.11&&12443.06&866.25&&14325.06\\
&&&\texttt{ADT}&&5.38&&810.39&182.30&&\bestvalue{9095.98}&\bestvalue{646.15}&&\bestvalue{10734.82}\\
&&&\texttt{RS}&&\bestvalue{4.93}&&5107.98&444.35&&9598.71&657.93&&15808.97\\
\arrayrulecolor{black!20}\hline\arrayrulecolor{black}
\multicolumn{2}{@{}l@{}}{learnresult\_fix}&&$\lsharp$&&5.51&&2079.48&454.47&&390.57&30.01&&2954.53\\
&&&$\lsharp_{\Ads}$&&5.99&&\bestvalue{1509.48}&\bestvalue{297.97}&&444.18&34.43&&\bestvalue{2286.06}\\
$n$ = 9&$k$ = 15&&\texttt{TTT}&&6.55&&2308.32&499.74&&678.86&49.17&&3536.09\\
&&&\texttt{ADT}&&5.81&&2538.33&394.99&&562.09&38.64&&3534.05\\
&&&\texttt{RS}&&\bestvalue{3.21}&&4298.31&321.66&&\bestvalue{118.97}&\bestvalue{8.88}&&4747.82\\
\arrayrulecolor{black!20}\hline\arrayrulecolor{black}
\multicolumn{2}{@{}l@{}}{OpenSSL\_1.0.1g\_client\_regular}&&$\lsharp$&&7.67&&991.53&219.06&&5585.07&397.77&&7193.43\\
&&&$\lsharp_{\Ads}$&&8.04&&\bestvalue{467.24}&\bestvalue{105.21}&&5436.12&386.92&&6395.49\\
$n$ = 10&$k$ = 7&&\texttt{TTT}&&5.94&&636.29&154.00&&4711.84&328.12&&\bestvalue{5830.25}\\
&&&\texttt{ADT}&&6.41&&860.05&164.77&&4908.55&347.64&&6281.01\\
&&&\texttt{RS}&&\bestvalue{4.98}&&3033.12&288.41&&\bestvalue{2684.53}&\bestvalue{191.09}&&6197.15\\
\arrayrulecolor{black!20}\hline\arrayrulecolor{black}
\multicolumn{2}{@{}l@{}}{OpenSSL\_1.0.1l\_server\_regular}&&$\lsharp$&&6.29&&905.66&220.06&&21326.23&1410.80&&23862.75\\
&&&$\lsharp_{\Ads}$&&6.78&&636.09&\bestvalue{145.03}&&22191.25&1478.07&&24450.44\\
$n$ = 10&$k$ = 7&&\texttt{TTT}&&6.76&&\bestvalue{600.41}&158.58&&21566.25&1438.12&&\bestvalue{23763.36}\\
&&&\texttt{ADT}&&6.19&&754.49&147.60&&23622.86&1567.63&&26092.58\\
&&&\texttt{RS}&&\bestvalue{6.08}&&3955.93&364.30&&\bestvalue{20465.68}&\bestvalue{1370.96}&&26156.87\\
\arrayrulecolor{black!20}\hline\arrayrulecolor{black}
\multicolumn{2}{@{}l@{}}{OpenSSL\_1.0.1j\_server\_regular}&&$\lsharp$&&6.36&&1059.33&241.40&&\bestvalue{24161.17}&\bestvalue{1571.78}&&\bestvalue{27033.68}\\
&&&$\lsharp_{\Ads}$&&6.77&&\bestvalue{699.95}&\bestvalue{150.75}&&28120.44&1819.17&&30790.31\\
$n$ = 11&$k$ = 7&&\texttt{TTT}&&7.13&&705.32&175.21&&30815.09&2001.78&&33697.40\\
&&&\texttt{ADT}&&6.56&&898.62&158.96&&25157.72&1638.99&&27854.29\\
&&&\texttt{RS}&&\bestvalue{6.15}&&4808.87&402.85&&28722.31&1856.74&&35790.77\\
\arrayrulecolor{black!20}\hline\arrayrulecolor{black}
\multicolumn{2}{@{}l@{}}{GnuTLS\_3.3.8\_client\_regular}&&$\lsharp$&&9.54&&1364.90&303.80&&451324.32&27124.13&&480117.15\\
&&&$\lsharp_{\Ads}$&&9.56&&\bestvalue{535.86}&\bestvalue{125.91}&&\bestvalue{429999.75}&\bestvalue{25849.52}&&\bestvalue{456511.04}\\
$n$ = 11&$k$ = 8&&\texttt{TTT}&&\bestvalue{9.23}&&987.33&230.63&&462575.01&27776.77&&491569.74\\
&&&\texttt{ADT}&&9.27&&1148.95&205.48&&466411.19&28009.34&&495774.96\\
&&&\texttt{RS}&&9.73&&8984.35&770.60&&451463.11&27105.14&&488323.20\\
\arrayrulecolor{black!20}\hline\arrayrulecolor{black}
\multicolumn{2}{@{}l@{}}{NSS\_3.17.4\_client\_full}&&$\lsharp$&&7.31&&2078.19&453.81&&\bestvalue{32498.93}&\bestvalue{2145.23}&&\bestvalue{37176.16}\\
&&&$\lsharp_{\Ads}$&&8.34&&\bestvalue{902.46}&\bestvalue{200.46}&&40699.57&2705.91&&44508.40\\
$n$ = 11&$k$ = 12&&\texttt{TTT}&&\bestvalue{6.70}&&965.71&254.42&&84864.87&5507.70&&91592.70\\
&&&\texttt{ADT}&&6.96&&1051.96&221.48&&105782.28&6698.76&&113754.48\\
&&&\texttt{RS}&&6.91&&9754.23&796.31&&60972.89&3990.11&&75513.54\\
\arrayrulecolor{black!20}\hline\arrayrulecolor{black}
\multicolumn{2}{@{}l@{}}{GnuTLS\_3.3.8\_server\_regular}&&$\lsharp$&&9.25&&1571.72&355.04&&136623.93&8584.27&&147134.96\\
&&&$\lsharp_{\Ads}$&&9.35&&\bestvalue{581.97}&\bestvalue{134.48}&&129102.33&8128.54&&137947.32\\
$n$ = 12&$k$ = 8&&\texttt{TTT}&&8.60&&914.31&225.65&&157839.22&9885.96&&168865.14\\
&&&\texttt{ADT}&&8.09&&1104.10&205.97&&145767.53&9164.61&&156242.21\\
&&&\texttt{RS}&&\bestvalue{7.50}&&7770.50&634.80&&\bestvalue{67966.55}&\bestvalue{4357.96}&&\bestvalue{80729.81}\\
\arrayrulecolor{black!20}\hline\arrayrulecolor{black}
\multicolumn{2}{@{}l@{}}{TCP\_FreeBSD\_Client}&&$\lsharp$&&6.92&&2289.74&492.68&&11267.74&778.03&&14828.19\\
&&&$\lsharp_{\Ads}$&&6.77&&\bestvalue{1132.21}&\bestvalue{239.65}&&11605.24&799.53&&13776.63\\
$n$ = 12&$k$ = 10&&\texttt{TTT}&&6.78&&2015.94&446.30&&9501.69&653.10&&12617.03\\
&&&\texttt{ADT}&&5.85&&1819.95&296.72&&9543.45&654.37&&\bestvalue{12314.49}\\
&&&\texttt{RS}&&\bestvalue{5.41}&&6982.82&550.39&&\bestvalue{8233.50}&\bestvalue{554.58}&&16321.29\\
\bottomrule
\end{tabular}


==> table_full_4.tex <==
% Warning: do not edit this file manually!
%
%
\begin{tabular}{@{}@{}l@{\hspace{1mm}}l@{}c@{}l@{}c@{}r@{}c@{}r@{\hspace{1mm}}r@{}c@{}r@{\hspace{1mm}}r@{}c@{}r@{}@{}}
\toprule%
\multicolumn{2}{@{}l@{}}{Model}
&\hspace*{2mm}&
\multicolumn{1}{@{}l@{}}{Algo-}
&\hspace*{2mm}&
\multicolumn{1}{@{}l@{}}{}
&\hspace*{2mm}&
\multicolumn{2}{@{}l@{}}{Learn-}
&\hspace*{2mm}&
\multicolumn{2}{@{}l@{}}{Test-}
&\hspace*{2mm}&
\multicolumn{1}{@{}l@{}}{}
\\
\cline{1-2}
%
%
\cline{8-9}
\cline{11-12}
%
\\[-4pt]
$n$
&
$k$
&
&
rithm
&
&
EQs
&
&
Inputs
&
Resets
&
&
Inputs
&
Resets
&
&
Total
\\
\midrule
\multicolumn{2}{@{}l@{}}{TCP\_Windows8\_Client}&&$\lsharp$&&\bestvalue{5.66}&&2537.64&520.59&&\bestvalue{7698.67}&\bestvalue{527.57}&&\bestvalue{11284.47}\\
&&&$\lsharp_{\Ads}$&&6.50&&\bestvalue{1504.24}&\bestvalue{279.52}&&9831.82&672.51&&12288.09\\
$n$ = 13&$k$ = 10&&\texttt{TTT}&&7.98&&2085.67&442.94&&15383.47&1045.90&&18957.98\\
&&&\texttt{ADT}&&7.58&&2818.29&421.76&&9039.31&631.45&&12910.81\\
&&&\texttt{RS}&&6.42&&9128.32&725.32&&8719.31&598.27&&19171.22\\
\arrayrulecolor{black!20}\hline\arrayrulecolor{black}
\multicolumn{2}{@{}l@{}}{TCP\_Linux\_Client}&&$\lsharp$&&8.86&&3095.37&646.31&&41814.35&2710.85&&48266.88\\
&&&$\lsharp_{\Ads}$&&9.47&&\bestvalue{1728.00}&\bestvalue{336.20}&&43672.28&2842.91&&48579.39\\
$n$ = 15&$k$ = 10&&\texttt{TTT}&&8.50&&3147.93&645.35&&\bestvalue{39448.46}&\bestvalue{2576.82}&&\bestvalue{45818.56}\\
&&&\texttt{ADT}&&8.92&&3230.09&481.57&&58246.62&3776.20&&65734.48\\
&&&\texttt{RS}&&\bestvalue{7.23}&&12872.18&956.92&&40579.28&2644.20&&57052.58\\
\arrayrulecolor{black!20}\hline\arrayrulecolor{black}
\multicolumn{2}{@{}l@{}}{GnuTLS\_3.3.8\_client\_full}&&$\lsharp$&&12.71&&3695.29&790.48&&2118359.37&128248.24&&2251093.38\\
&&&$\lsharp_{\Ads}$&&12.74&&\bestvalue{1107.82}&\bestvalue{248.56}&&2183860.24&132530.08&&2317746.70\\
$n$ = 15&$k$ = 12&&\texttt{TTT}&&12.64&&2052.11&473.23&&2160486.33&130945.24&&2293956.91\\
&&&\texttt{ADT}&&\bestvalue{11.70}&&1969.34&378.96&&2406607.40&145753.37&&2554709.07\\
&&&\texttt{RS}&&11.74&&22354.29&1926.29&&\bestvalue{1891570.94}&\bestvalue{114696.03}&&\bestvalue{2030547.55}\\
\arrayrulecolor{black!20}\hline\arrayrulecolor{black}
\multicolumn{2}{@{}l@{}}{OpenSSL\_1.0.1g\_server\_regular}&&$\lsharp$&&8.56&&1872.45&394.68&&37720.47&2384.62&&42372.22\\
&&&$\lsharp_{\Ads}$&&9.83&&\bestvalue{1161.84}&235.21&&38480.72&2447.14&&42324.91\\
$n$ = 16&$k$ = 7&&\texttt{TTT}&&9.03&&1473.41&331.58&&42366.02&2690.85&&46861.86\\
&&&\texttt{ADT}&&7.61&&1274.51&\bestvalue{230.77}&&\bestvalue{31678.33}&\bestvalue{2013.93}&&\bestvalue{35197.54}\\
&&&\texttt{RS}&&\bestvalue{6.29}&&6823.62&598.54&&42989.03&2677.14&&53088.33\\
\arrayrulecolor{black!20}\hline\arrayrulecolor{black}
\multicolumn{2}{@{}l@{}}{GnuTLS\_3.3.8\_server\_full}&&$\lsharp$&&12.00&&3663.81&774.90&&555275.27&34664.72&&594378.70\\
&&&$\lsharp_{\Ads}$&&11.55&&\bestvalue{1123.95}&\bestvalue{248.00}&&472976.53&29498.93&&503847.41\\
$n$ = 16&$k$ = 11&&\texttt{TTT}&&11.32&&1756.95&418.20&&506809.47&31735.75&&540720.37\\
&&&\texttt{ADT}&&10.77&&1827.97&335.26&&539188.33&33643.54&&574995.10\\
&&&\texttt{RS}&&\bestvalue{10.15}&&20495.94&1617.38&&\bestvalue{346658.16}&\bestvalue{21869.93}&&\bestvalue{390641.41}\\
\arrayrulecolor{black!20}\hline\arrayrulecolor{black}
\multicolumn{2}{@{}l@{}}{DropBear}&&$\lsharp$&&9.20&&5283.63&870.11&&34251.78&2166.16&&42571.68\\
&&&$\lsharp_{\Ads}$&&11.98&&\bestvalue{3411.55}&\bestvalue{553.86}&&29448.29&1904.79&&35318.49\\
$n$ = 17&$k$ = 13&&\texttt{TTT}&&11.86&&5372.69&905.68&&33573.63&2171.21&&42023.21\\
&&&\texttt{ADT}&&10.36&&4122.24&617.36&&25764.85&1678.13&&\bestvalue{32182.58}\\
&&&\texttt{RS}&&\bestvalue{6.59}&&17666.79&1258.94&&\bestvalue{13306.88}&\bestvalue{866.19}&&33098.80\\
\arrayrulecolor{black!20}\hline\arrayrulecolor{black}
\multicolumn{2}{@{}l@{}}{OpenSSH}&&$\lsharp$&&19.79&&25058.68&3907.52&&\bestvalue{1420810.47}&\bestvalue{80721.84}&&\bestvalue{1530498.51}\\
&&&$\lsharp_{\Ads}$&&21.93&&\bestvalue{10783.46}&\bestvalue{1665.03}&&1517837.57&86105.79&&1616391.85\\
$n$ = 31&$k$ = 22&&\texttt{TTT}&&18.48&&14408.62&2487.83&&2106605.28&119174.68&&2242676.41\\
&&&\texttt{ADT}&&17.53&&13826.78&1874.73&&1953538.60&110583.56&&2079823.67\\
&&&\texttt{RS}&&\bestvalue{10.69}&&104984.85&6635.57&&1747643.65&98694.50&&1957958.57\\
\arrayrulecolor{black!20}\hline\arrayrulecolor{black}
\multicolumn{2}{@{}l@{}}{model4}&&$\lsharp$&&19.68&&28731.52&3827.40&&27858.50&1325.21&&61742.63\\
&&&$\lsharp_{\Ads}$&&22.41&&18868.28&1868.44&&28438.01&1368.67&&\bestvalue{50543.40}\\
$n$ = 34&$k$ = 14&&\texttt{TTT}&&21.09&&18864.22&2793.27&&32723.10&1589.43&&55970.02\\
&&&\texttt{ADT}&&20.92&&\bestvalue{18008.41}&\bestvalue{1505.27}&&34826.25&1647.89&&55987.82\\
&&&\texttt{RS}&&\bestvalue{11.08}&&77936.81&4842.28&&\bestvalue{8359.44}&\bestvalue{403.81}&&91542.34\\
\arrayrulecolor{black!20}\hline\arrayrulecolor{black}
\multicolumn{2}{@{}l@{}}{model1}&&$\lsharp$&&7.78&&9679.96&1308.49&&10548.64&655.90&&22192.99\\
&&&$\lsharp_{\Ads}$&&7.85&&\bestvalue{6832.78}&\bestvalue{794.71}&&11622.10&724.60&&\bestvalue{19974.19}\\
$n$ = 35&$k$ = 15&&\texttt{TTT}&&11.77&&9879.92&1681.13&&11402.54&713.65&&23677.24\\
&&&\texttt{ADT}&&8.94&&8410.19&1159.94&&11852.78&733.03&&22155.94\\
&&&\texttt{RS}&&\bestvalue{4.85}&&31513.88&2046.84&&\bestvalue{1959.90}&\bestvalue{133.42}&&35654.04\\
\arrayrulecolor{black!20}\hline\arrayrulecolor{black}
\multicolumn{2}{@{}l@{}}{TCP\_Windows8\_Server}&&$\lsharp$&&23.16&&27848.73&3247.90&&506861.24&28256.37&&566214.24\\
&&&$\lsharp_{\Ads}$&&24.12&&\bestvalue{17035.46}&\bestvalue{1789.66}&&481803.64&26983.07&&527611.83\\
$n$ = 38&$k$ = 13&&\texttt{TTT}&&27.49&&19998.26&2579.75&&554970.20&30983.03&&608531.24\\
&&&\texttt{ADT}&&24.63&&19062.25&1839.28&&522854.14&29153.41&&572909.08\\
&&&\texttt{RS}&&\bestvalue{11.22}&&88537.94&5074.22&&\bestvalue{140818.07}&\bestvalue{7964.42}&&\bestvalue{242394.65}\\
\arrayrulecolor{black!20}\hline\arrayrulecolor{black}
\multicolumn{2}{@{}l@{}}{TCP\_FreeBSD\_Server}&&$\lsharp$&&30.41&&53430.17&5201.33&&786916.89&41169.88&&886718.27\\
&&&$\lsharp_{\Ads}$&&34.67&&\bestvalue{28090.92}&\bestvalue{2528.64}&&880079.60&45874.76&&956573.92\\
$n$ = 55&$k$ = 13&&\texttt{TTT}&&35.49&&34650.97&3621.54&&668327.57&35255.36&&741855.44\\
&&&\texttt{ADT}&&33.79&&32968.56&2622.59&&751184.96&39159.92&&825936.03\\
&&&\texttt{RS}&&\bestvalue{14.56}&&176695.43&9733.47&&\bestvalue{444159.86}&\bestvalue{23210.48}&&\bestvalue{653799.24}\\
\bottomrule
\end{tabular}


==> table_full_5.tex <==
% Warning: do not edit this file manually!
%
%
\begin{tabular}{@{}@{}l@{\hspace{1mm}}l@{}c@{}l@{}c@{}r@{}c@{}r@{\hspace{1mm}}r@{}c@{}r@{\hspace{1mm}}r@{}c@{}r@{}@{}}
\toprule%
\multicolumn{2}{@{}l@{}}{Model}
&\hspace*{2mm}&
\multicolumn{1}{@{}l@{}}{Algo-}
&\hspace*{2mm}&
\multicolumn{1}{@{}l@{}}{}
&\hspace*{2mm}&
\multicolumn{2}{@{}l@{}}{Learn-}
&\hspace*{2mm}&
\multicolumn{2}{@{}l@{}}{Test-}
&\hspace*{2mm}&
\multicolumn{1}{@{}l@{}}{}
\\
\cline{1-2}
%
%
\cline{8-9}
\cline{11-12}
%
\\[-4pt]
$n$
&
$k$
&
&
rithm
&
&
EQs
&
&
Inputs
&
Resets
&
&
Inputs
&
Resets
&
&
Total
\\
\midrule
\multicolumn{2}{@{}l@{}}{TCP\_Linux\_Server}&&$\lsharp$&&31.89&&48035.66&4795.18&&821110.22&43285.08&&917226.14\\
&&&$\lsharp_{\Ads}$&&36.95&&\bestvalue{27730.98}&2514.78&&785883.53&41525.04&&857654.33\\
$n$ = 57&$k$ = 12&&\texttt{TTT}&&35.24&&35176.91&3759.52&&794674.37&41833.81&&875444.61\\
&&&\texttt{ADT}&&34.38&&29541.56&\bestvalue{2380.81}&&918691.24&48389.22&&999002.83\\
&&&\texttt{RS}&&\bestvalue{14.72}&&169782.62&9407.62&&\bestvalue{291075.22}&\bestvalue{15466.60}&&\bestvalue{485732.06}\\
\arrayrulecolor{black!20}\hline\arrayrulecolor{black}
\multicolumn{2}{@{}l@{}}{model3}&&$\lsharp$&&22.24&&60706.81&7347.66&&43379.00&2684.39&&114117.86\\
&&&$\lsharp_{\Ads}$&&26.37&&33990.69&3703.85&&52503.04&3245.99&&\bestvalue{93443.57}\\
$n$ = 58&$k$ = 22&&\texttt{TTT}&&26.24&&35771.47&5205.59&&58231.15&3576.05&&102784.26\\
&&&\texttt{ADT}&&26.67&&\bestvalue{33035.42}&\bestvalue{3160.37}&&57865.50&3561.65&&97622.94\\
&&&\texttt{RS}&&\bestvalue{12.14}&&215860.78&14273.09&&\bestvalue{16613.11}&\bestvalue{1019.75}&&247766.73\\
\arrayrulecolor{black!20}\hline\arrayrulecolor{black}
\multicolumn{2}{@{}l@{}}{BitVise}&&$\lsharp$&&33.03&&44794.28&4499.48&&2306551.51&120942.82&&\bestvalue{2476788.09}\\
&&&$\lsharp_{\Ads}$&&39.47&&\bestvalue{26910.45}&2404.41&&2809658.31&146435.51&&2985408.68\\
$n$ = 66&$k$ = 13&&\texttt{TTT}&&42.13&&43145.21&3977.16&&2559975.40&134109.12&&2741206.89\\
&&&\texttt{ADT}&&37.30&&27293.16&\bestvalue{2365.21}&&2975447.04&153177.77&&3158283.18\\
&&&\texttt{RS}&&\bestvalue{17.47}&&223860.20&14090.38&&\bestvalue{2300385.66}&\bestvalue{118905.61}&&2657241.85\\
\bottomrule
\end{tabular}

